Efficient Computation of General Modules for ALC Ontologies (Extended Version)

We present a method for extracting general modules for ontologies formulated in the description logic ALC. A module for an ontology is an ideally substantially smaller ontology that preserves all entailments for a user-specified set of terms. As such, it has applications such as ontology reuse and ontology analysis. Different from classical modules, general modules may use axioms not explicitly present in the input ontology, which allows for additional conciseness. So far, general modules have only been investigated for lightweight description logics. We present the first work that considers the more expressive description logic ALC. In particular, our contribution is a new method based on uniform interpolation supported by some new theoretical results. Our evaluation indicates that our general modules are often smaller than classical modules and uniform interpolants computed by the state-of-the-art, and compared with uniform interpolants, can be computed in a significantly shorter time. Moreover, our method can be used for, and in fact improves, the computation of uniform interpolants and classical modules.

==> computing_UT.tex <==
\section{Computing Uniform Interpolant via $\texttt{rolE}_\Sigma$}
From $\texttt{conE}_{\Sigma}(\texttt{rolE}_\Sigma(\OsplitForm))$, one sometimes can compute a
uniform interpolant for $\mathcal{O}$ and $\Sigma$ similarly as in
\cite{koopmann2020lethe}.
%\patrick{In what follows, you state that this is indeed not the case. One can
%only \emph{sometimes} compute a uniform interpolant.}
%\hui{corrected}
In brief, the uniform interpolant for $\mathcal{O}$
and $\Sigma$ is generated from  $\texttt{conE}_{\Sigma}(\texttt{rolE}_\Sigma(\OsplitForm))$ by the following  two
steps:
\begin{enumerate}
    \item Apply the resolution rule \emph{D-Res} in Figure \ref{fig:UI-rule} exhaustively;
    \item Delete all clauses containing definers.
\end{enumerate}
Note that Step 1 terminates iff no axiom of the form $\neg D_1\sqcup Q r. C\sqcup C_1$, where $D_1\in\sig(C)$, could be generated.  In this case, we can obtain a new ontology denoted as $U(\Omc, \Sigma)$.  we have the following result:
\begin{theorem}\label{theo:UI}
Let $\Sigma$ be a signature, and let $\mathcal{O}$ be an
$\mathcal{ALC}$-ontology. If $U(\Omc, \Sigma)$
 exists, then we have $U(\Omc, \Sigma)$
is a uniform interpolant for $\mathcal{O}$ and $\Sigma$.
\end{theorem}



\begin{figure}
    \centering
   \begin{tcolorbox}
       \emph{D-Res}:
   \begin{equation}\nonumber
      \frac{C_1\sqcup Q r. D_1, \bigcup\limits_{j=2}^{n}\{ C_j\sqcup \forall r.
D_j\},\bigcup\limits_{i=1}^{k}\{N_i\sqcup C_i'\}}{C_1\sqcup \cdots\sqcup
C_n\sqcup Q r. (C_1'\sqcap\cdots\sqcap C_k')},
    \end{equation}
    where  (i) $Q\in \{\forall, \exists\}$; (ii) $N_i = \sqcup_{j\in
I_i} \neg D_j$ for some $I_i\subseteq \{1, 2, \cdots, n\}$; (iii) $C_i'$ do not contain negative definers. 
    \end{tcolorbox}
    \caption{Resolution rule: \emph{D-Res}}
    \label{fig:UI-rule}
\end{figure}

\begin{example}[Example \ref{exp:con_elimination} continued]
By applying D-Res rule in
$\texttt{conE}_{\Sigma}(\texttt{rolE}_\Sigma(\OsplitForm)
)$, we obtain a uniform interpolant for $\mathcal{O}$ and $\Sigma$:
 $$U(\Omc, \Sigma) = \{\neg A_1\sqcup \exists r. (\neg A_2\sqcup A_3) \sqcup
\exists r. A_4\}.$$
\end{example} 
However, \emph{D-Res} may
generate axioms of the form $\neg D_1\sqcup Q r. C\sqcup C_1$, where $D_1\in\sig(C)$ (even if a uniform interpolant  exists).
%\patrick{Careful here: this sentence almost sounds like whether the uniform
%interpolant exists can be determined using \emph{D-Res}. I doubt that this is
%the case.}
%\hui{Yes, it is not the case. I modified it to avoid confusion}
Here is an
example.%Then $U(\Omc, \Sigma)$ is not a uniform interpolant anymore.
\begin{example}\label{exp:exp_loop}
Let $\Sigma = \{A, A_1, r, s\}$ and $$\mathcal{O} = \{A\sqsubseteq \exists r.B,\  B\sqsubseteq \exists s. B,\  B\sqsubseteq B_1,\   B_1\sqsubseteq A_1\}.$$ 
\begin{align*}
    cl(\mathcal{O}) =\{&\neg A\sqcup \exists r. D_1,\ \neg D_1\sqcup B,\  B\sqsubseteq \exists s. D_2,\\
    &\neg D_2\sqcup B,\  \neg B\sqcup B_1,\ \neg B_1 \sqcup A_1\}.
\end{align*}
Then the axiom $\neg D_2\sqcup \exists s. D_2$ is in the ontology 
\begin{align*}
  \texttt{conE}_{\Sigma}(\texttt{rolE}_{\Sigma}&(\OsplitForm))=\{\neg A\sqcup \exists r. D_1,\ \neg D_1\sqcup \exists s. D_2\\
    &\neg D_1\sqcup A_1,\ \neg D_2\sqcup \exists s. D_2, \neg D_2\sqcup A_1\}.
\end{align*}
\end{example}

However, no matter a uniform interpolant exists or not, we could always compute
an new ontology $U_{ap}(\Omc, \Sigma)$ by substitute the occurrence of $D_1$ in  $\neg D_1\sqcup Q r.
C \sqcup C_1$ ($D_1\in\sig(C)$) to $C_{D_1}$ when applying rule D-Res.
\begin{example}[Example \ref{exp:exp_loop} continued]
By replacing $D_2$ to $C_{D_2}=B$, we obtain $U_{ap}(\Omc, \Sigma)=$
\begin{align*}
 \{\neg A\sqcup \exists r. (\exists s. B\sqcap A_1),\  \neg B\sqcup \exists s. B,\ \neg B \sqcup A_1\}.
\end{align*}
It is not a uniform interpolant for $\Omc^1$ and $\Sigma^1$ because it contains
a concept name $B\not\in \Sigma^1$, which is introduced by replacing $D_2$ to
$C_{D_2}$.
\end{example}

$U_{ap}(\Omc, \Sigma)$ is an approximate uniform interpolant because
of the following result:
\begin{theorem}
Let $\Sigma$ be a signature, and let $\mathcal{O}$ be an
$\mathcal{ALC}$-ontology. Then we have $U_{ap}(\Omc, \Sigma)\equiv_\Sigma
\Omc$.
\end{theorem}

Different from the general module $gm(\Omc, \Sigma)$, which allows $C_D$ that may contain names outside given signature, $U_{ap}(\Omc, \Sigma)$ aims  to eliminates names outside given signature $\Sigma$ as much as possible using rule D-Res. 
Depending on the situation, we may have $|U_{ap}(\Omc, \Sigma)|\leq |gm(\Omc, \Sigma)|$ or otherwise. 
However, computing $U_{ap}(\Omc, \Sigma)$ from $\texttt{conE}_{\Sigma}(\texttt{rolE}_\Sigma(\OsplitForm))$ could take exponential times or more wrt. the size of $\texttt{conE}_{\Sigma}(\texttt{rolE}_\Sigma(\OsplitForm))$, but  $gm(\Omc, \Sigma)$ only take a linear time.

%For instance, in Example \ref{exp:general_mod}, we have $$U_{ap}(\Omc, \Sigma) = \{A_1\sqsubseteq\exists r.(\neg A_2\sqcup A_3)\sqcup\exists r.A_4\},$$
%which is more concise than $gm(\Omc, \Sigma)$. 
%However, $|U_{ap}(\Omc, \Sigma)|$  could be exponential to the size of  $|\texttt{conE}_{\Sigma\cup
%\textsf{N}_D}(\texttt{rolE}_\Sigma(\OsplitForm))|$, which is equal to $|gm(\Omc, \Sigma)| $.
%Moreover, 


==> preprocessing.tex <==
\section{Preprocessing}\label{sec:preprocess}
As stated in Section \ref{sec:sigmaForm}, we pre-compute $\mathcal{S}$ (see
Lemma \ref{theo-preprocessing}) for the given ontology $\Omc$ to accelerate the
role isolation process producing $\OsplitForm$.
However, in the worst case, $\mathcal{S}$ may contain exponentially many axioms
(wrt $\lvert\cl(\Omc)\rvert$) and thus its computation may be
time-consuming even with the method from
Lemma~\ref{theo-preprocessing}.

To overcome this difficulty, we consider $\mathcal{S}$ as the union
$\cup_{r\in \sig(\Omc)} \mathcal{S}^r$, where $\mathcal{S}^r\subseteq
\mathcal{S}$ is the subset  of all axioms $\neg D_1\sqcup \ldots\sqcup
\neg D_n$ such that $r\in \Rol(D_i, cl(\Omc))$, $1\leq i \neq n$.
This decomposition allows us to  compute $\mathcal{S}^r$ for each
$r\in\sig(\Omc)$.
The computation of $\mathcal{S}^r$ itself is accelerated by extracting a \starM\
for the signature $\Sigma_r =\{D\in \sig(\cl(\Omc))\mid r\in \Rol(D,
\cl(\Omc))\}$ over $\cl(\Omc)$.

Note that, if $\Sigma\subseteq \Sigma_0$, then by definition any general module
$\gm_{\Sigma_0}(\Omc)$ is also a general module for $\Omc$ and $\Sigma$.
Suppose some component $\mathcal{S}^r$ cannot be computed due to time or
space limitations. We can still obtain a general module for $\Omc$ and
$\Sigma$ by extending $\Sigma$ to $\Sigma\cup \{r\}$. 
\patrick{And how do you use this fact? Do you extend $\Sigma$ in your
implementation based on a timeout parameter? Something is missing in this
section.}
\hui{Yes, we  extend $\Sigma$ based on a timeout parameter. This only make sense if we do not consider the time cost of preprocessing step.

If we consider the total time containing preprocessing time, then these paragraph make no sense. In this case, we can delete this section and move the statement of computation of $S^r$ the next paragraph of Lemma 1.
}
